Josephson oscillations of edge solitons in a photonic-topological coupler

We introduce a scheme of a photonic coupler built of two parallel topological-insulator slab waveguides with the intrinsic Kerr nonlinearity, separated by a gap. Josephson oscillations (JO) of a single edge soliton created in one slab, and of a pair of solitons created in two slabs, are considered. The single soliton jumping between the slabs is subject to quick radiative decay. On the other hand, the JO of the copropagating soliton pair may be essentially more robust, as one soliton can absorb dispersive waves emitted by the other. The most robust JO regime is featured by the pair of solitons with phase shift $\pi$ between them.

==> frequency.tex <==
\begin{figure}[tbh]
\centering
\includegraphics[width=1\linewidth]{Figs/jumping-distance.eps}
\caption{The period of quasi-soliton's JO (Josephson oscillations), $T_{1/2}$, vs.
width $\Delta $ of the lattice spacing separating the lattice slabs formimg the coupler.
Values of $\Delta $ are shown in units of the lattice spacing, $d$. (a) The
results for the JO of a single quasi-soliton, which was initially created in one
slab. (b) The results for the pair of quasi-solitons initially created in two
slabs, with phase difference $\Delta \protect\phi (0)$ between them. \textcolor{purple}{The points are joined by arbitrary lines for convenience.} }
\label{fig:jumping-distance}
\end{figure}

We define the oscillation period, $T_{1/2}\equiv z_{2}-z_{1}$, as the distance
between the first two consecutive points, $z_{1}$ and $z_{2}$, at which the
numerical solution exhibits equal energies in both waveguiding slabs. The
oscillations are not strictly periodic because the period is affected by the
continuing energy loss. Only values $T_{1/2}>0.1$ cm were registered, as
smaller ones may be a result of fluctuations caused by the interaction of
the quasi-solitons with the dispersive waves.

First, we consider JO initiated by the single quasi-soliton, launched at $z=0$ in
one waveguiding slab. Depending on the lattice spacing width, the initial quasi-soliton
performs the oscillations periodically jumping across the lattice spacing, whose width
is smaller than a critical value $\Delta _{\mathrm{cr}}$, which takes values
$1.1d\leq \Delta _{\mathrm{cr}}\leq 1.2d$ (recall $d$ is the lattice
spacing). At $\Delta >\Delta _{\mathrm{cr}}$, the quasi-soliton stays in its
initial slab. Thus, JO performed by the single quasi-soliton are characterized by
the dependence of the JO period, $T_{1/2}$, on $\Delta $, which is presented
in Fig. \ref{fig:jumping-distance}(a), in the interval of $0.6d\leq \Delta
\leq 1.1d$ (for $\Delta \leq 0.5d$ the two lattice slabs start to touch each
other, closing the lattice spacing between them, while at $\Delta >1.1d$ the proximity
to $\Delta _{\mathrm{cr}}$ makes $T_{1/2}$ extremely large).

Next, Fig. \ref{fig:jumping-distance}(b) summarizes the results produced by
the simulations of JO of two edge solitons which were initially created in
the two slabs, with phase difference $\Delta \phi (0)$. It is seen that the
JO frequency, $2\pi /T_{1/2}$, attains a maximum at $\Delta \phi (0)=\pi $
and a minimum at $\Delta \phi (0)=0$. This observation is explained by the
fact that the solitons repel and attract each other in the former and latter
cases, respectively \cite{RMP}, hence the respective interaction force
accelerates or decelerates the mutual motion of the solitons. Indeed, a full
picture of the simulated evolution shows that the quasi-solitons periodically pass
through each other, thus shuttling between the opposite slabs, or bounce
back from each other, thus oscillating between one slab and the lattice spacing
midplane, in the cases of $\Delta \phi (0)=0$ and $\pi $, respectively. Case $\Delta\phi(0)=\pi/2$  corresponds to inelastic bouncing with strong energy exchange   between the edge quasi-solitons.
Further, it is observed that the period of two-quasi-soliton JO naturally
increases approximately linearly with the increase of the lattice spacing width $
\Delta$. \textcolor{purple}{We have varified, that in linear case the frequency of Josephson oscillations doesn't depend on the initial phase difference at all. As expected, in the linear case, the wave packets and Josephson oscillations decay much faster than for the nonlinear lattice. }

\textcolor{purple}{Remarkably,  the half-period functions in Fig. \ref{fig:jumping-distance}(b) are quite similar for cases $\Delta \phi (0)=\pi$ and $\Delta \phi (0)=\pi/2$. This symmetry is explained by the nonlinearity which breaks usual symmetry for two antiphase quasisolions. 
%The cases of $\Delta \phi (0)=\pi/2$ and $\Delta \phi %(0)=3\pi/2$ differ by the relative sign of the two %quasi-solitons. 
}
%($\pi$ corresponds to factor -1)



